On the Geometry of Conullity Two Manifolds

If $\Gamma$ is the nullity space of the curvature tensor of a Riemannian manifold $M^n$, it is well known that if its dimension is constant and if $M^n$ is complete then the distribution $\Gamma$ is completely integrable with flat leaves. The case of $\dim \Gamma = n-2$ are the so called conullity two manifolds which naturally arise in various geometric contexts. The obstruction to the metric splitting isometrically is a 2x2 matrix which is either nilpotent or invertible. We study the case where it is nilpotent, or equivalently where the scalar curvature is constant along the leaves of $\Gamma$. When $M^n$ is locally irreducible we show that $M^n$ admits a Lipschitz foliation $F$ by totally geodesic flat hyperplanes and determine the metric on a naturally defined open dense subset in terms of $n-1$ functions, uniquely determined up to isometry. We can also find examples of smooth complete metrics of conullity two where the foliation $F$ is smooth only on the complement of a Cantor set. We furthermore show that the fundamental group is either trivial or infinite cyclic.

==> sections/app_curvscal.tex <==
% !TEX root = ../Conull2Notes.tex

\section{Curvature depends only on the scalar curvature} \label{app:scalgivesR}
It turns out that if we have conullity two then the curvature is entirely determined by the sectional curvature of the plane orthogonal to the nullity.
To see why the curvature tensor is determined by the scalar curvature, recall that knowledge of the sectional curvature of any plane determines the entire curvature tensor. 
Letting \(T_1, \dots, T_{n}\) be orthonormal nullity vectors and \(e_1, e_2\) be orthonormal vectors in the plane orthogonal to the nullity, we can describe any plane as the span of two vectors
\begin{align}
v_1 &= a_1 T_1 + \dots + a_{n} T_{n} + a_{n+1} e_1 + a_{n+2} e_2; \\
v_2 &= b_1 T_1 + \dots + b_{n} T_{n} + b_{n+1} e_1 + b_{n+2} e_2,
\end{align}
where
\begin{equation}
\sum_{i = 1}^{n+2} a_i^2 = \sum_{i=1}^{n+2} b_i^2 = 1.
\end{equation}
Let \(x = \expval{a,b} = a_1b_1 + \dots + a_{n+2} b_{n+2}\). 
Then we have
\begin{align}
\sec(v_1, v_2) &= \frac{R(v_1, v_2, v_2, v_1)}{1-x^2} \nonumber \\
&= \frac{R(a_{n+1} e_1, b_{n+2} e_2, b_{n+1} e_1, a_{n+2} e_2)}{1-x^2} + \frac{R(a_{n+1} e_1, b_{n+2} e_2, b_{n+2} e_2, a_{n+1} e_1)}{1-x^2} \nonumber \\
&+ \frac{R(a_{n+2} e_2, b_{n+1} e_1, b_{n+1} e_1, a_{n+2} e_2)}{1-x^2} + \frac{R(a_{n+2} e_2, b_{n+1} e_1, b_{n+2} e_2, a_{n+1} e_1)}{1-x^2} \nonumber \\
&= \frac{a_{n+1}^2 b_{n+2}^2 - 2 a_{n+1} a_{n+2} b_{n+1} b_{n+2} + a_{n+2}^2 b_{n+1}^2}{1-x^2} R(e_1, e_2, e_2, e_1) \nonumber \\
&= \frac{(a_{n+1}b_{n+2} - a_{n+2} b_{n+1})^2}{1-x^2} \sec(e_1, e_2).
\end{align}
Thus the sectional curvature of an arbitrary plane is determined by the sectional curvature of the \(e_1e_2\) plane and by the coordinates of the plane with respect to the basis. 


==> sections/app_metriccomps.tex <==
% !TEX root = ../Conull2Notes.tex

\section{Computations from section \ref{sec:metric}}\label{app:metriccomps}

\begin{lem}\label{lem:Ainverse}
If we have a symmetric square matrix
\begin{equation} \label{eq:Amatrixform}
A = \begin{pmatrix}
	\bfun^2 + b_2^2 + b_3^2 + \dots + b_{n}^2 & b_2 & b_3 & \cdots & b_{n} \\
	b_2 & 1 & 0 & \cdots & 0 \\
	b_3 & 0 & 1 & \cdots & 0 \\
	\vdots & \vdots & \vdots & \ddots & \vdots \\
	b_{n} & 0 & 0 & \cdots & 1
	\end{pmatrix}
\end{equation}
then the inverse is given by the symmetric matrix
\begin{equation}
A^{-1} = \frac{1}{\bfun^2} \begin{pmatrix}
	1 & -b_2 & -b_3 & \cdots & -b_{n} \\
	-b_2 & & & & \\
	-b_3 & & & & \\
	\vdots & & & a_{ij} & \\
	-b_{n} & & & &
	\end{pmatrix}
\end{equation}
where for \(i, j \geq 2\),
\begin{equation}
a_{ij} = \begin{cases} \bfun^2 + b_i^2 & i = j, \\
b_i b_j & i \neq j.
\end{cases}
\end{equation}
\end{lem}

\begin{proof}
One may check this by multiplying a row in \(A\) by a column in the proposed \(A^{-1}\). Since most rows and columns in \(A\) and \(A^{-1}\) follow a pattern, with the first in each being the only exception, one can do this with finitely many checks.
\end{proof}

\begin{cor}\label{cor:invcomps}
The inverse to the metric \eqref{eq:bmetric} has components
\begin{align}
g^{xx} = \frac{1}{\bfun^2}, \quad g^{x\uu} = -\frac{g_{x\uu}}{\bfun^2}, \quad g^{x\vv{i}} = -\frac{g_{x\vv{i}}}{\bfun^2}, \quad g^{\uu \uu} = \frac{\bfun^2 + g_{\uu \uu}^2}{\bfun^2}, \\
g^{\uu \vv{i}} = \frac{g_{x \uu} g_{x \vv{i}}}{\bfun^2}, \quad g^{\vv{i} \vv{i}} = \frac{\bfun^2 + g_{x \vv{i}}^2}{\bfun^2}, \quad g^{\vv{i}\vv{j}} = \frac{g_{x \vv{i}} g_{x \vv{j}}}{\bfun^2}. \nonumber
\end{align}
\end{cor}

\begin{proof}
The metric in \eqref{eq:bmetric} has a matrix form which is of the form of \ref{eq:Amatrixform} and hence Lemma \ref{lem:Ainverse} tells us what the form of the inverse is. 
These are just what the lemma tells us the components of the inverse are. 
\end{proof}

In order to verify the properties of the metric \eqref{eq:bmetric} we need to compute many Christoffel symbols using the formula
\begin{equation}
\Gamma_{ij}^k = \frac{1}{2} g^{k\ell} \left(\pdv{g_{i\ell}}{x_j} + \pdv{g_{j\ell}}{x_i} - \pdv{g_{ij}}{x_\ell}\right).
\end{equation}

To verify \ref{eq:christxu} we compute
\begin{equation}
\Gamma_{x \uu}^\placedot = \christ{x}{\uu}{\placedot}.
\end{equation}
Now if \(\ell = x\) then we have the second two terms in the parentheses cancelling out leaving only
\begin{align*}
\frac{1}{2} g^{\placedot x} \pdv{g_{xx}}{\uu} &= \frac{1}{2} g^{\placedot x} \pdv{\uu} \left(\bfun(x,\uu)^2 + \sum_{j=0}^n (\vv{j-1} f_j(x) - \vv{j+1}f_{j+1}(x))^2 \right) \\
&= \frac{1}{2} g^{\placedot x} \left(2\bfun \bfun_{\uu} + 2f_1(x)(\uu f_1(x) - \vv{2} f_2(x))\right) \\
&= g^{\placedot x} (\bfun \bfun_{\uu} + f_1(x)(\uu f_1(x) - \vv{2} f_2(x))).
\end{align*}

If \(\ell = \uu\) then the first and third terms cancel out and we are left with
\begin{equation*}
\frac{1}{2} g^{\placedot \uu} \pdv{g_{\uu \uu}}{x} = \frac{1}{2} g^{\placedot \uu} \pdv{x}(1) = 0.
\end{equation*}

If \(\ell = \vv{1}\) then the middle term is zero as \(g_{\uu \vv{1}} = 0\), while the other terms are nonzero:
\begin{equation*}
\frac{1}{2} g^{\placedot \vv{1}} \left( \pdv{g_{x \vv{1}}}{\uu} - \pdv{g_{x \uu}}{\vv{1}}\right) = \frac{1}{2} g^{\placedot \vv{1}} (f_1(x) - (-f_1(x))) = g^{\placedot \vv{1}} f_1(x).
\end{equation*}

Lastly, if \(\ell = \vv{i}\) for \(i \geq 2\) then all the derivatives vanish.
Adding these parts together gives 
\begin{equation*}
\Gamma_{x \uu}^\placedot = g^{\placedot x}(\bfun \bfun_u + f_1 (\uu f_1(x) - \vv{2} f_2(x))) + g^{\placedot \vv{1}} f_1
\end{equation*}
as stated in \ref{eq:christxu}.

To verify \ref{eq:christxvi} we compute
\begin{equation}
\Gamma_{x \vv{i}}^\placedot = \christ{x}{\vv{i}}{\placedot}.
\end{equation}
If we take \(\ell = x\) then the second two terms cancel and we are left with
\begin{align*}
\frac{1}{2} g^{\placedot x} \pdv{g_{xx}}{\vv{i}} &= \frac{1}{2} g^{\placedot x} \pdv{\vv{i}} \left(\bfun(x,\uu)^2 + \sum_{j=0}^n (\vv{j-1} f_j(x) - \vv{j+1}f_{j+1}(x))^2 \right) \\
&=  \frac{1}{2} g^{\placedot x} \pdv{\vv{i}} \left((\vv{i-2} f_{i-1}(x) - \vv{i}f_i(x))^2 + (\vv{i} f_{i+1}(x) - \vv{i+2}f_{i+2}(x))^2 \right) \\
&= g^{\placedot x} (-f_i(x) g_{x \vv{i-1}} + f_{i+1}(x) g_{x \vv{i+1}}).
\end{align*}

Now if we take \(\ell = \vv{i-1}\) (here we treat \(\uu = \vv{0}\) for brevity's sake) then the middle term is zero and we have
\begin{equation*}
\frac{1}{2} g^{\placedot \vv{i-1}} \left(\pdv{g_{x \vv{i-1}}}{\vv{i}} - \pdv{g_{x\vv{i}}}{\vv{i-1}}\right) = \frac{1}{2} g^{\placedot \vv{i-1}} (-f_i(x) - f_i(x)) = -g^{\placedot \vv{i-1}} f_i(x),
\end{equation*}
while if we take \(\ell = \vv{i+1}\) then the middle term is again zero and we have
\begin{equation*}
\frac{1}{2} g^{\placedot \vv{i+1}} \left(\pdv{g_{x \vv{i+1}}}{\vv{i}} - \pdv{g_{x\vv{i}}}{\vv{i+1}}\right) = \frac{1}{2} g^{\placedot \vv{i+1}} (f_{i+1}(x) - (-f_{i+1}(x))) = g^{\placedot \vv{i+1}} f_{i+1}(x).
\end{equation*}
Finally if we take \(\ell\) to be anything else every term vanishes so taking these together we get
\begin{equation*}
\Gamma_{x \vv{i}}^\placedot = g^{\placedot x}(-f_i g_{x \vv{i-1}} + f_{i+1} g_{x \vv{i+1}}) - g^{\placedot \vv{i-1}} f_i + g^{\placedot \vv{i+1}} f_{i+1}
\end{equation*}
as claimed.

To verify that the other symbols \(\Gamma_{\uu \uu}^\placedot\), \(\Gamma_{\uu \vv{i}}^\placedot\), and \(\Gamma_{\vv{i} \vv{j}}^\placedot\) are all zero as claimed in \ref{eq:christuu} we compute
\begin{equation}
\Gamma_{\uu \uu}^\placedot = \christ{\uu}{\uu}{\placedot}.
\end{equation}
However there is no component \(g_{\uu \ell}\) which depends on \(\uu\) and \(g_{\uu \uu}\) is a constant so this is zero.
Similarly,
\begin{equation}
\Gamma_{\uu \vv{i}}^\placedot = \christ{\uu}{\vv{i}}{\placedot}.
\end{equation}
The only way any terms are nonzero here are if \(i = 1\) and \(\ell = x\), but then computing this gives 
\begin{equation*}
\frac{1}{2} g^{\placedot x}\left(\pdv{g_{\uu x}}{\vv{1}} + \pdv{g_{\vv{1} x}}{\uu}\right) = \frac{1}{2} g^{\placedot x} (-f_1(x) + f_1(x)) = 0.
\end{equation*}
Therefore this is always zero.
Lastly, looking at
\begin{equation}
\Gamma_{\vv{i} \vv{j}}^\placedot = \christ{\vv{i}}{\vv{j}}{\placedot},
\end{equation}
the only hope of a nonzero term lies with taking \(\ell = x\) and \(j = i + 1\) (or \(i - 1\) but then we can swap \(i\) and \(j\)).
Then similarly to before we get
\begin{equation*}
\Gamma_{\vv{i} \vv{i+1}}^\placedot = \frac{1}{2}g^{\placedot x}(-f_{i+1}(x) + f_{i+1}(x)) = 0,
\end{equation*}
and so this symbol is zero as well.

To verify \ref{item:nullity} and \ref{item:scal} from \ref{lem:bfunmetricprops} we need to do computations. 
We can compute the Christoffel symbols as
\begin{align}
	\Gamma_{x \uu}^\placedot &= g^{\placedot x}(\bfun \bfun_u + f_1 g_{x \vv{1}}) + g^{\placedot \vv{1}} f_1, \label{eq:christxu}\\
	\Gamma_{x \vv{i}}^\placedot &= g^{\placedot x}(-f_i g_{x \vv{i-1}} + f_{i+1} g_{x \vv{i+1}}) - g^{\placedot \vv{i-1}} f_i + g^{\placedot \vv{i+1}} f_{i+1}, \label{eq:christxvi} \\
	\Gamma_{\uu \uu}^\placedot &= \Gamma_{\uu \vv{i}}^\placedot = \Gamma_{\vv{i}\vv{j}}^\placedot = 0. \label{eq:christuu}
\end{align}
From here we may compute the components of the curvature tensor. 

In order to show that all \(\pdv{\vv{i}}\) are nullity vectors it suffices to show that \(R(\bullet, \bullet)\pdv{\vv{i}} = 0\). 
Furthermore, from the Christoffel symbols we see that \(\nabla_{\pdv{\uu}} \pdv{\vv{i}} = 0\) and hence it suffices to check that
\begin{equation*}
	R\left(\pdv{\uu}, \pdv{x}\right) \pdv{v_i} = 0 \quad \text{and} \quad R\left(\pdv{\vv{j}}, \pdv{x}\right) \pdv{v_i} = 0.
\end{equation*}
To that end we compute all components \(R_{\uu x \vv{i}}^\bullet\) and \(R_{\vv{j} x \vv{i}}^\bullet\) and using the Christoffel symbols above we find that they are all zero as desired. 
Hence they are in fact nullity vectors. 

Finally to show the curvature, since all \(\pdv{v_i}\) are nullity vectors, the scalar curvature is twice the sectional curvature of the orthogonal plane. 
In other words, it is twice the sectional curvature of \(\orthvect\) and \(\pdv{\uu}\). 
\begin{align}
	\scal &= 2 \sec(\orthvect, \pdv{\uu}) = 2 R\left(\orthvect, \pdv{\uu}, \pdv{\uu}, e_2\right) = 2R \left(\frac{1}{\bfun} \pdv{x}, \pdv{\uu}, \pdv{\uu}, \frac{1}{\bfun} \pdv{x}\right) \nonumber \\
	&= \frac{2}{\bfun^2} R\left(\pdv{x},\pdv{\uu}, \pdv{\uu}, \pdv{x}\right).
\end{align}
Therefore it suffices to show that \(R\left(\pdv{x},\pdv{\uu}, \pdv{\uu}, \pdv{x}\right) = -\bfun \bfun_{\uu \uu}\).

Doing the computations we find that
\begin{align}
	R_{x \uu \uu}^x &= -\frac{\bfun_{\uu \uu}}{\bfun} \\
	R_{x \uu \uu}^\uu &= g_{x \uu} \frac{\bfun_{\uu \uu}}{\bfun} \\
	R_{x \uu \uu}^{\vv{i}} &= g_{x \vv{i}} \frac{\bfun_{\uu \uu}}{\bfun}.
\end{align}
Then we have
\begin{align}
	R\left(\pdv{x},\pdv{\uu}, \pdv{\uu}, \pdv{x}\right) &= R_{x \uu \uu}^x g_{xx} + R_{x \uu \uu}^\uu g_{\uu x} + \sum_i R_{x \uu \uu}^{\vv{i}} g_{\vv{i} x} \nonumber \\
	&= -\frac{\bfun_{\uu \uu}}{\bfun} (\bfun^2 + g_{x \uu}^2 + \sum_i g_{x \vv{i}}^2) + g_{x \uu}^2 \frac{\bfun_{\uu \uu}}{\bfun} + \sum_i g_{x \vv{i}}^2 \frac{\bfun_{\uu \uu}}{\bfun} \nonumber \\
	&= - \bfun \bfun_{\uu \uu},
\end{align}
as desired.
Hence the curvature is as claimed.

For \ref{item:a1def} recall that we already know that the nullity \(\Gamma\) is given by the span of the \(\pdv{\vv{i}}\), and therefore the orthogonal complement to the nullity \(\Gamma^\perp\) is given by the span of \(\left\{\pdv{\uu}, \orthvect \right\}\).
Therefore we need to show the following:
\begin{equation*}
	\nabla_u \pdv{\vv{i}} = 0. \quad \left(\nabla_{\orthvect} \pdv{\vv{1}}\right)^{\Gamma^\perp} = -a_1 \pdv{\uu}. \quad  \left(\nabla_{\orthvect} \pdv{\vv{i}}\right)^{\Gamma^\perp} = 0 \; (i \geq 2).
\end{equation*}
The first of these follows immediately from the fact that \(\Gamma_{\uu \vv{i}}^\placedot = 0\).
Since it is also true that \(\Gamma_{\vv{i} \vv{j}}^\placedot = 0\), the only term in the expression for \(\orthvect\) that matters when it comes to these derivatives is the \(\frac{1}{\bfun} \pdv{x}\) term.
Hence
\begin{equation*}
	\nabla_{\orthvect} \pdv{\vv{1}} = \nabla_{\frac{1}{\bfun} \pdv{x}} \pdv{\vv{1}} = \frac{1}{\bfun} \nabla_{x} \pdv{\vv{1}} = \frac{1}{\bfun} \Gamma_{x \vv{1}}^\placedot \pdv{\placedot}.
\end{equation*}
But one may check that the only \(\Gamma_{x \vv{1}}^\placedot\) which are nonzero are
\begin{equation*}
	\Gamma_{x \vv{1}}^{\uu} = -f_1 \quad \text{and} \quad \Gamma_{x \vv{1}}^{\vv{2}} = f_2.
\end{equation*}
so
\begin{equation}\label{eq:v1derivative}
	\nabla_{\orthvect}\pdv{\vv{1}} = -\frac{f_1(x)}{\bfun(x,\uu)}\pdv{\uu} + \frac{f_2(x)}{\bfun(x,\uu)}\pdv{\vv{2}}
\end{equation}
which after projecting gives
\begin{equation}
	\left(\nabla_{\orthvect}\pdv{\vv{1}}\right)^{\Gamma^\perp} = -\frac{f_1(x)}{\bfun(x,\uu)} \pdv{\uu}.
\end{equation}
This shows that indeed \(a_1 = \frac{f_1(x)}{\bfun(x,\uu)}\) as claimed.

Lastly we need to check that \(\left(\nabla_{\orthvect} \pdv{\vv{i}}\right)^{\Gamma^\perp} = 0\). 
This is done similarly to the previous case, where we note that the only nonzero \(\Gamma_{x \vv{i}}^\placedot\) terms are
\begin{equation*}
	\Gamma_{x \vv{i}}^{\vv{i-1}} = -f_i \quad \text{and} \quad \Gamma_{x \vv{i}}^{\vv{i+1}} = f_{i+1}.
\end{equation*}
which gives
\begin{equation}\label{eq:viderivative}
	\nabla_{\orthvect}\pdv{\vv{i}} = -\frac{f_{i}(x)}{\bfun(x,\uu)}\pdv{\vv{i-1}} + \frac{f_{i+1}(x)}{\bfun(x,\uu)}\pdv{\vv{i+1}}.
\end{equation}
However, both of their corresponding terms are killed upon projecting, and therefore these derivatives are zero.
These computations show that indeed \(\orthvect\), \(\pdv{\uu}\), and \(\pdv{\vv{1}}\) play the roles of \(e_2\), \(e_2\), and \(T_1\) in the splitting tensor argument as claimed.

For the Frenet vectors we observe that \ref{eq:v1derivative} tells us that \(T_2 = \pdv{\vv{2}}\) and \(a_2(x,\uu,\vv{i}) = \frac{f_2(x)}{\bfun(x,\uu)}\).
Then \ref{eq:viderivative} inductively gives us that this is true for larger \(i\) as well.

For \(\beta\) we may again use the computations of the Christoffel symbols to reach the result by computing it as \(\expval{\nabla_{e_2} \pdv{\uu}, e_2}\), but it can also be derived from \ref{eq:1overa1jacobi} which says that \(\beta = -a_1 e_1\left(\frac{1}{a_1}\right)\).

For \ref{item:leavesxconst} recall that the leaves of this foliation are given by flowing in the directions of \(\pdv{\uu}\) and \(\pdv{\vv{i}}\).
The leaves are clearly hyperplanes from the dimension.
Since Christoffel symbols of the form \(\Gamma_{\uu \uu}^\placedot\) and \(\Gamma_{\vv{i} \vv{i}}^\placedot\) are zero it follows that the integral curves along these coordinate vector fields are geodesics and therefore gives the leaves, so \(x\) is constant on each leaf. 



==> sections/app_onmanifold.tex <==
% !TEX root = ../Conull2Notes.tex

\section{Verifying the computations to get the metric on the manifold}
Here we check that the coordinate vectors are indeed the \( e_1 \) and \( T_i \) vectors as claimed. 
At some point \(p = (x,\uu, \vv{i})\) we have that
\begin{align}
	\pdv{x}\eval_p &= \dd(\exp_{\gamma(x)})_{(\uu e_1 + \vv{i} T_i)} (e_2),\\
	\pdv{\uu}\eval_p &= \dd(\exp_{\gamma(x)})_{(\uu e_1 + \vv{i} T_i)} (e_1),\\
	\pdv{\vv{i}}\eval_p &= \dd(\exp_{\gamma(x)})_{(\uu e_1 + \vv{i} T_i)} (T_i).
\end{align}
To determine what these are we use Jacobi fields along the geodesic \(\rho\) defined by \(\rho(0) = \gamma(x)\) and \(\rho'(0) = {\uu} e_1 + {\vv{i}} T_i\).
Since the leaves of \(\mathcal{F}\) are flat and totally geodesic,  \(\rho\) lives in one leaf. 
In the case of \(\pdv{\uu}\), take the Jacobi field such that \(J(0) = 0\) and \(\dot{J}(0) = e_1\). 
Since the initial conditions of our Jacobi field and \(\rho\) are in a single flat totally geodesic leaf of \(\mathcal{F}\), it follows that the curvature term of the Jacobi equation vanishes, \(J(t) = te_1\), and so  \(\pdv{\uu}\) is the same thing as parallel translating \(e_1\) from \(\gamma(x)\) along the geodesic \(\exp_{\gamma(x)}(t({\uu} e_1 + {\vv{i}} T_i))\), and likewise the same conclusion holds for \(\pdv{\vv{i}}\) and \(T_i\).

Earlier calculations showed \(\nabla_T T_1 = 0\), \(\nabla_{e_1} T_1 = 0\), and \(\nabla_T e_1 = 0\) for any \(T \in \Gamma\), so parallel translation along \( T \) preserves \(T_1\) and \(e_1\) as defined by the splitting tensor, and hence \(\pdv{\uu} = e_1\) and \(\pdv{\vv{1}} = T_1.\) 
Likewise since \(\nabla_T T_i = 0\) and \(\nabla_{e_1} T_i = 0\) we conclude that \(T_i = \pdv{\vv{i}}\) for \(i \geq 2\) as well.

When we computed \( \pdv{\phi}{x} \) we computed a Jacobi field by
\begin{align}
	J'(0) &= \frac{D}{\dd s} \pdv{\alpha_s}{t} \eval_{s=0, t=0} \\
	&= \nabla_{e_2}({\uu} e_1 + {\vv{i}} T_i) \nonumber \\
	&= {\uu}(a_1 T_1 - \beta e_2) + {\vv{i}} \nabla_{e_2}T_i \nonumber \\
	&= {\uu}(a_1 T_1 - \beta e_2) + {\vv{1}}(-a e_1 + a_2 T_2) \nonumber \\
	& \quad + \sum_{i=2}^{n-1} {\vv{i}} (-a_i T_{i-1} + a_{i+1}T_{i+1}) - {\vv{n}} a_{n} T_{n-1} \nonumber \\
	&= -{\uu} \beta e_2 - a_1 {\vv{1}} e_1 + ({\uu} a_1 - {\vv{2}} a_2) T_1 \nonumber \\
	& \quad + \sum_{i=2}^{n-1} ({\vv{i-1}}a_i - {\vv{i+1}}a_{i+1})T_i +  {\vv{n-1}} a_{n} T_{n}. \nonumber
\end{align}

==> sections/app_prelimcomps.tex <==
% !TEX root = ../Conull2Notes.tex

\section{Computations from section \ref{sec:prelim}} \label{app:prelimcomps}
To check equation \ref{eq:scalprime} we have
\begin{align} \label{eq:scalprimemore}
\scal' &= 2\expval{(\nabla_T R)(e_1, e_2)e_2, e_1} 
\\ &= -2 \expval{(\nabla_{e_1} R)(e_2, T) e_2, e_1} - 2\expval{(\nabla_{e_2}R)(T, e_1) e_2, e_1} \nonumber \\
&= 2\expval{R(e_2,\nabla_{e_1}T)e_2, e_1} + 2\expval{R(\nabla_{e_2}T, e_1) e_2, e_1} \nonumber \\
&= -2 \expval{R(e_2,C_T(e_1))e_2, e_1} - 2\expval{R(C_T(e_2), e_1) e_2, e_1} \nonumber \\
&= (\expval{C_T(e_1),e_1} + \expval{C_T(e_2),e_2}) \scal \nonumber \\
&= \tr(C_T) \scal. \nonumber
\end{align}

To verify \ref{eq:curvcomp122}, we have
\begin{align}
R(e_1, e_2) e_2 &= \riem{e_1}{e_2}{e_2} \\
&= \nabla_{e_1}(\beta e_1) - \nabla_{e_2}(-\alpha e_1) + \alpha \nabla_{e_1}e_2 + a_1 \nabla_{T_1}e_2 - \beta \nabla_{e_2} e_2 \nonumber \\
&= (e_1(\beta) + e_2(\alpha) - \alpha^2 - \beta^2)e_1 + (\alpha\beta - \alpha \beta) e_2 + \alpha a_1 T_1 \nonumber \\
&= \alpha a_1 T_1 + (e_1(\beta) + e_2(\alpha) - \alpha^2 - \beta^2)e_1. \nonumber
\end{align}

To verify \ref{eq:curvcomp211} we have
\begin{align}
R(e_2, e_1)e_1 &= \riem{e_2}{e_1}{e_1} \\
&= - \nabla_{e_1}(a_1 T_1 - \beta e_2) - a_1 \nabla_{T_1} e_1 + \beta \nabla_{e_2} e_1 \nonumber \\
&= -e_1(a_1)T_1 - a_1 \nabla_{e_1}T_1 + e_1(\beta)e_2 + \beta (a_1 T_1 - \beta e_2) \nonumber \\
&= (a_1 \beta - e_1(a_1))T_1 - a_1 \nabla_{e_1}T_1 + (e_1(\beta) - \beta^2)e_2. \nonumber
\end{align}

To verify \ref{eq:curvcompT21}, we have
\begin{align}
R(T, e_2)e_1 &= \riem{T}{e_2}{e_1} \\
&= \nabla_T (a_1 T_1 - \beta e_2) - \nabla_{e_2}(-f_1 e_2) - f_1 \nabla_{e_1} e_1 + f_2 \nabla_{\tilde{T}} e_1 \nonumber \\
&= T(a_1) T_1 + a_1 \nabla_T T_1 - T(\beta) e_2 - \beta \nabla_T e_2 + e_2(f_1) e_2 + f_1 \nabla_{e_2}e_2 + f_2 \nabla_{\tilde{T}}e_1 \nonumber \\
&= T(a_1) T_1 + a_1 \nabla_T T_1 + (-f_1 \beta + f_1 \beta)e_1 + (e_2(f_1) - T(\beta))e_2 + f_2 \nabla_{\tilde{T}}e_1. \nonumber
\end{align}

To verify \ref{eq:curvcomp1TT1} we denote \(\nabla_{e_1}T = \delta \tilde{T}\) and then we have
\begin{align}
R(e_1, T)T_1 &= \riem{e_1}{T}{T_1} \\
&= 0 - 0 - \delta \nabla_{\tilde{T}}T_1 - f_1 \nabla_{e_2} T_1 \nonumber \\
&= - f_1 \nabla_{e_2}T_1. \nonumber
\end{align}

To verify \ref{eq:curvcompt121}, say that \(\nabla_{e_2} T_1 = -a_1 e_1 + \delta \tilde{T}\), and so we have
\begin{align}
R(T_1, e_2)e_1 &= \riem{T_1}{e_2}{e_1} \\
&= \nabla_{T_1} (a_1 T_1 - \beta e_2) + 0 - a_1 \nabla_{e_1} e_1 + \delta \nabla_{\tilde{T}} e_1 \nonumber \\
&= T_1(a_1) T_1 + a_1 \nabla_{T_1}T_1 - T_1(\beta) e_2. \nonumber
\end{align}

To verify \ref{eq:curvcomp12T1} we compute
\begin{align}
R(e_1, e_2) T_1 &= \riem{e_1}{e_2}{T_1} \\
&= \nabla_{e_1}(-a_1 e_1 + a_2 T_2) - \beta (-a_1 e_1 + a_2 T_2) \nonumber \\
&= -e_1(a_1) e_1 + e_1(a_2) T_2 + a_2 \nabla_{e_1} T_2 + a_1 \beta e_1 - a_2 \beta T_2 \nonumber \\
&= (a_1 \beta - e_1(a_1)) e_1 + (e_1(a_2) - a_2 \beta) T_2 + a_2 \nabla_{e_1}T_2 \nonumber \\
&= (e_1(a_2) - a_2 \beta) T_2 + a_2 \nabla_{e_1}T_2. \nonumber
\end{align}

To verify \ref{eq:curvcompT12T1} we compute
\begin{align}
R(T_1, e_2)T_1 &= \riem{T_1}{e_2}{T_1} \\
&= \nabla_{T_1}(-a_1 e_1 + a_2 T_2) + a_2 \nabla_{T_2} T_1 \nonumber \\
&= -T_1(a_1)e_1 + T_1(a_2)T_2 + a_2 \nabla_{T_1}T_2. \nonumber
\end{align}

To verify \ref{eq:curvcompT2T1} we compute
\begin{align}
R(T, e_2)T_1 &= \riem{T}{e_2}{T_1} \\
&= \nabla_{T}(-a_1 e_1 + a_2 T_2) \nonumber \\
&= -T(a_1) e_1 + T(a_2) T_2 + a_2 \nabla_T T_2. \nonumber
\end{align}

To verify \ref{eq:curvcomp12Ti} we compute
\begin{align}
R(e_1, e_2) T_i &= \riem{e_1}{e_2}{T_i} \\
&= \nabla_{e_1}(-a_i T_{i-1} + a_{i+1} T_{i+1}) - \beta (-a_i T_{i-1} + a_{i+1} T_{i+1}) \nonumber \\
&= -e_1(a_i) T_{i-1} + a_{i+1}\nabla_{e_1}T_{i+1} + e_1(a_{i+1}) T_{i+1} + a_i \beta T_{i-1} - a_{i+1}\beta T_{i+1} \nonumber \\
&= (a_i \beta - e_1(a_i)) T_{i-1} + (e_1(a_{i+1}) - a_{i+1}\beta)T_{i+1} + a_{i+1} \nabla_{e_1} T_{i+1} \nonumber \\
&= (e_1(a_{i+1}) - a_{i+1}\beta)T_{i+1} + a_{i+1} \nabla_{e_1} T_{i+1}. \nonumber
\end{align}

To verify \ref{eq:curvcompT12Ti} we compute
\begin{align}
R(T_1, e_2)T_i &= \riem{T_1}{e_2}{T_i} \\
&= \nabla_{T_1}(-a_i T_{i-1} + a_{i+1} T_{i+1}) + a_2 \nabla_{T_2} T_i \nonumber \\
&= -T_1(a_i) T_{i-1} - a_i \nabla_{T_1}T_{i-1} + T_1(a_{i+1})T_{i+1} + a_{i+1} \nabla_{T_1} T_{i+1} \nonumber \\
&= T_1(a_{i+1})T_{i+1} + a_{i+1} \nabla_{T_1} T_{i+1}. \nonumber
\end{align}

To verify \ref{eq:curvcompT2Ti} we compute
\begin{align}
R(T, e_2)T_i &= \riem{T}{e_2}{T_i} \\
&= \nabla_{T}(-a_i T_{i-1} + a_{i+1} T_{i+1}) \nonumber \\
&= T(a_{i+1})T_{i+1} + a_{i+1} \nabla_T T_{i+1}. \nonumber
\end{align}



